Graph-based Global Robot Simultaneous Localization and Mapping using Architectural Plans

In this paper, we propose a solution for graph-based global robot simultaneous localization and mapping (SLAM) using architectural plans. Before the start of the robot operation, the previously available architectural plan of the building is converted into our proposed architectural graph (A-Graph). When the robot starts its operation, it uses its onboard LIDAR and odometry to carry out an online SLAM relying on our situational graph (S-Graph), which includes both, a representation of the environment with multiple levels of abstractions, such as walls or rooms, and their relationships, as well as the robot poses with their associated keyframes. Our novel graph-to-graph matching method is used to relate the aforementioned S-Graph and A-Graph, which are aligned and merged, resulting in our novel informed Situational Graph (iS-Graph). Our iS-Graph not only provides graph-based global robot localization, but it extends the graph-based SLAM capabilities of the S-Graph by incorporating into it the prior knowledge of the environment existing in the architectural plan

==> related_works.tex <==
\section{Related Work}
\label{related_works}
% \subsection{Global Localization}

% Global localization refers to the estimation of the pose of a robot on a known map. Global localization is usually done in two steps. Initial localization is usually performed by sensor-reading-to-map matching~\cite{majdik2013mav,kim2017satellite}, which is frequently referred to as \emph{re-localization}~\cite{kendall2016modelling}, \emph{place recognition}~\cite{lowry2015visual} or \emph{the kidnapped robot prolem}~\cite{desrochers2015set}. After an initial pose has been estimated within the known map, the robot pose is tracked in such map fusing its dynamics and sensor readings.

% Multiple sensor modalities, including LiDAR~\cite{miller2021any}, monocular~\cite{leung2008localization}, and stereo~\cite{zuo2020multimodal} cameras, can be employed for such tasks. Fox et al.~\cite{Markov-Loc} proposed one of the pioneer works in global localization, in which they use a Markov model to update with each sensor reading, a probability distribution over the space of potential locations in the surrounding environment. If the robot becomes confident about its location, the probability distribution converges to a single mode centered around the true position of the robot. Markov localization has, however, a high computational footprint. To overcome this issue, \cite{MCL} proposed Monte Carlo Localization (MCL), which models the robot state as a set of particles that are randomly sampled from the probability density function. MCL has proven to be effective in a wide variety of scenarios \cite{scan-MCL}, \cite{mpd-MCL}, \cite{ndt-mcl}.

% Hess et al.~\cite{cartographer} proposed Cartographer, a real-time indoor mapping algorithm along with localization capability. It uses submap based scan-matching technique for estimating the initial odometry. A global loop closure is performed to optimize the estimated trajectory and further improve the accuracy of the map. The localization-only mode of Cartographer then uses this map for global localization.

% Other methods rely on the extraction and matching of local point cloud descriptors such as \cite{fpfh}, \cite{sog}, \cite{bowpf}. Keypoint-based methods are constrained by the limited distinctiveness of local structures in LiDAR data. However, they have emerged as an alternative to those based on scan matching and have garnered significant interest from the research community in recent years \cite{fast_histo}, \cite{M2dp}.

% Recent research has shown some promising results in learning-based localization. \cite{seg-map} presented SegMap which creates a different map representation for localization by extracting segments from 3D point clouds. Most global localization approaches assume that the prior maps were estimated using the same sensors used for localization. This limits the use of maps estimated from other sensor modalities or human maps, as we do. As we are addressing this specific last case, we refer to related works in the next subsection.

\subsection{Localization in Architectural Plans}
Boniardi et al.~\cite{PGLOC-CADfloorPlans} proposed the use of CAD plans for robust LiDAR indoor localization. They first create a globally consistent sparse map by combining Bayes filtering and graph-based mapping techniques. The robot then estimates its pose in the global frame of the floor plan by aligning this map to the CAD plan. \cite{room-layout-edge-extraction} also proposed a localization approach in digital floor plans with a monocular camera. They predict the room layout by using a convolutional neural network (CNN) named room layout extraction network. Then they use a particle filter to estimate the robot pose by matching the extracted edges from the network and the digital floor plan. \cite{GLFP} performed global localization using schematic floor plans. They proposed a factor-graph-based localization approach that uses features --such as wall intersections and corners from the digital floor plans-- as landmarks. Their approach assumes that the features mentioned above are previously labeled. The robot extracts similar features from a 3D point cloud and performs data association. The robot poses and landmarks are jointly optimized by a factor graph. \cite{Precise-Robot-Localization-in-Architectural-3D-Plans} addressed the issue of localization in erroneous architectural plans. They first segment RGB images using a segmentation network into foreground and background, then fuse them with LiDAR scans. Then they perform local referencing to make up for the deviations in the digital plan and perform precise localization. They also proposed an outlier detector to counter noise and clutter in sensor readings. They claim that their method outperforms the Iterative Closest Point (ICP) based method by almost $30 \%$. \cite{SGD-LOC} also addressed localization in inaccurate floor plans using Stochastic Gradient Descent (SGD) and 2D LiDAR. They benchmark their algorithm against Adaptive Monte Carlo Localization (AMCL) \cite{AMCL} and claim to significantly outperform it in the case of imprecise maps. Ling et al.~\cite{FP-LOC} proposed a novel idea of Approximate Nearest Neighbor Fields (ANNF) which they use for localization on floor plans. ANNF allows for fast  retrieval of the closest geometric floor plan features for any point within the localization space. \cite{Towards-BIM-based-robot-localization} proposed to use of Building Information Modelling (BIM) for robot localization. Instead of using the traditional Simultaneous Localization and Mapping (SLAM) algorithm, they convert the BIM model to a localization-oriented point cloud and localize the robot using ICP between the robot's laser scanner and the metric point cloud. \cite{vega:2022:2DLidarLocalization} proposes an open-source method to generate appropriate Pose Graph-based maps from BIM models for robust 2D-LiDAR localization in changing and dynamic environments. They first create 2D occupancy grid maps automatically from BIM (Building Information Modelling) and then convert them into Pose-Graph-based maps. Then using various map representations they perform localization using different localization algorithms. \cite{BIM-LOC} explore an effective way to localize a mobile 3D LiDAR sensor on BIM-generated maps considering both geometric and semantic properties. 

\subsection{Graph Matching}

Several approaches have tackled the problem of associating data from two different sets. ~\cite{bailey2000data} formulates a maximum common sub-graph problem, or maximum clique when new noisy data is acquired incrementally. ~\cite{antonante2021outlier} performs an outlier-robust estimation, maximum consensus, and truncated least squares. CLIPPER ~\cite{lusk2021clipper} presents a relaxation of this NP-hard problem. They weigh the geometric consistency of different associations and encounter the most consistent associations (inliers) by finding the densest sub-graph, hence as a graph theoretic framework. The authors provide experiments with point and point-normal noisy sets with outliers. ~\cite{arandjelovic2016netvlad} use a convolutional neural network for large places recognition visually. 

The literature has approached the problem of graph matching for robot localization with a loop-closure goal. ~\cite{global_loc_gnn}  takes as input two graphs describing scenes. Random walks are accomplished in both of them generating class-aware descriptors of each walk. The node association is based on the number of identical descriptors in common. Distance comparison between nodes is used when ambiguity remains for different match candidates.~\cite{semantic_loop_closure} use a sparse Kuhn–Munkres algorithm to find the association between nodes of graphs extracted from images. The similarity is computed in terms of shape and image similitudes along the euclidian distance. ~\cite{zheng2020buildingfusion} measure the similarities by comparing the instance-level embeddings provided by 3D CNNs followed by a graph-wise geometrical verification.

The concept of 3D scene graphs for representing the structure of an environment in a hierarchical manner was introduced by \cite{scene_graph} and \cite{3d_scene_graph}.
~\cite{hydra} presented a hierarchical loop-closer detection in graphs. First, they compare descriptors in a top-down fashion to find putative loop closures at places, objects, and vision. Those descriptors contain statistics of the robot’s surroundings at object and place levels combining geometrical and semantic information. Both are aggregated as histograms for its comparison. Second, a bottom-up verification of the geometric consistency yields a match between robot nodes.
